Improved Approximation Algorithms for Three-Dimensional Knapsack

We study the three-dimensional Knapsack (3DK) problem, in which we are given a set of axis-aligned cuboids with associated profits and an axis-aligned cube knapsack. The objective is to find a non-overlapping axis-aligned packing (by translation) of the maximum profit subset of cuboids into the cube. The previous best approximation algorithm is due to Diedrich, Harren, Jansen, Th\"{o}le, and Thomas (2008), who gave a $(7+\varepsilon)$-approximation algorithm for 3DK and a $(5+\varepsilon)$-approximation algorithm for the variant when the items can be rotated by 90 degrees around any axis, for any constant $\varepsilon>0$. Chleb\'{\i}k and Chleb\'{\i}kov\'{a} (2009) showed that the problem does not admit an asymptotic polynomial-time approximation scheme. We provide an improved polynomial-time $(139/29+\varepsilon) \approx 4.794$-approximation algorithm for 3DK and $(30/7+\varepsilon) \approx 4.286$-approximation when rotations by 90 degrees are allowed. We also provide improved approximation algorithms for several variants such as the cardinality case (when all items have the same profit) and uniform profit-density case (when the profit of an item is equal to its volume). Our key technical contribution is container packing -- a structured packing in 3D such that all items are assigned into a constant number of containers, and each container is packed using a specific strategy based on its type. We first show the existence of highly profitable container packings. Thereafter, we show that one can find near-optimal container packing efficiently using a variant of the Generalized Assignment Problem (GAP).

==> LPs.tex <==
\section{Proving the approximation ratios}
In this section, we aim to show the approximation ratio that result from the algorithm we provide. We do this by using linear programming to find the optimal approximation ratio given for each case.  We further provide the dual of each linear program to prove that the approximation ratio is bounded as we desire.

We begin showing the approximation ratios by showing the guarantees given when the volume of items that are none-large in the optimal solution is small. As a brief reminder, here are the guarantees we provide for this case.
\begin{align*}
    \alg &\ge \left(\frac{2}{3}-O(\epsilon)\right)\max\{\opt_1,\opt_2,\opt_3\} && [\text{\Cref{thm:structuredpackingalgo}}]\\
    \alg &\ge (1-O(\epsilon))\left(\opt_L+\max\{\alpha_1, \beta_1,\gamma_1\}\right) && [\text{\Cref{thm:big&largealgo}}]\\
    \alg &\ge (1-O(\epsilon))\left(\frac{3}{4}\alpha_1+\alpha_2\right) && [\text{\Cref{thm:packingI1}}]\\
    \alg &\ge (1-O(\epsilon))\left(\frac{3}{4}\beta_1+\beta_2\right) && [\text{\Cref{thm:packingI1}}]\\
    \alg &\ge (1-O(\epsilon))\left(\frac{3}{4}\gamma_1+\gamma_2\right) && [\text{\Cref{thm:packingI1}}]
\end{align*}
We can then transform these guarantees into a linear program. We omit the factors of $O(\varepsilon)$ as they can be linearly added to the final approximation ratio. The resulting primal LP is the following.

\begin{equation*}
    \begin{array}{rl}
    \text{minimize } & \alg \\
    \alg -\frac{2}{3}\opt_1 &\ge 0\\
    \alg -\frac{2}{3}\opt_2 &\ge 0\\
    \alg -\frac{2}{3}\opt_3 &\ge 0\\
    \alg -\opt_L+\alpha_1 &\ge 0\\
    \alg -\opt_L+\beta_1 &\ge 0\\
    \alg -\opt_L+\gamma_1 &\ge 0\\
    \alg -\frac{3}{4}\alpha_1- \alpha_2 &\ge 0\\
    \alg -\frac{3}{4}\beta_1- \beta_2 &\ge 0\\
    \alg -\frac{3}{4}\gamma_1- \gamma_2 &\ge 0\\
    \opt_1+\opt_2+\opt_3+\opt_L&= 1\\
    -\opt_1 +\alpha_1+ \alpha_2 &= 0\\
   -\opt_2 +\beta_1+ \beta_2 &= 0\\
    -\opt_3 +\beta_1+ \beta_2 &= 0\\    
    \end{array}
\end{equation*}

Here, the last four constraints ensure the integrity of the values of $\opt_1,\opt_2,\opt_3,\opt_L$ and $\alpha_1,\alpha_2$ ($\beta_1,\beta_2,\gamma_1,\gamma_2$ respectively). Furthermore, all variables are $\ge 0$. The optimal value of this LP is $\frac{1}{4}$, implying an approximation ratio of $\frac{1}{\frac{1}{4}}=4$. Adding in the factor of $O(\varepsilon)$ yields the final ratio of $4+O(\varepsilon)$. We show that this ratio is correct by providing a feasible assignment that yields an objective value of $\frac{1}{4}$ of the dual LP. After transforming the LP, the resulting dual LP is the following:

\begin{equation*}
    \begin{array}{rl}
    \text{maximize } & y_{10} \\
    y_1+y_2+y_3+y_4+y_5+y_6+y_7+y_8+y_9 &\le 1\\
    -\frac{2}{3}y_1+y_{10}-y_{11}&\le 0\\
    -\frac{2}{3}y_2+y_{10}-y_{12}&\le 0\\
    -\frac{2}{3}y_3+y_{10}-y_{13}&\le 0\\
    -y_4-y_5-y_6+y_{10}&\le 0\\
    -y_4-\frac{3}{4}y_7+y_{11}&\le 0\\
    -y_7+y_{11}&\le 0\\
    -y_5-\frac{3}{4}y_8+y_{12}&\le 0\\
    -y_8+y_{12}&\le 0\\
    -y_6-\frac{3}{4}y_9+y_{13}&\le 0\\
    -y_9+y_{13}&\le 0\\
    \end{array}
\end{equation*}

With $y_1,\dots,y_9 \ge 0, y_{10},\dots,y_{13}\in \mathbb{R}.$ Here, the indexes of the variable correspond to its related constraint in the primal LP. A feasible solution of this dual LP with objective value $\frac{1}{4}$ is given by:
\begin{align*}
    y_1 &= 0\\
    y_2 &= 0\\
    y_3 &= 0\\
    y_4 &= \frac{1}{16}\\
    y_5 &= \frac{1}{16}\\
    y_6 &= \frac{2}{16}\\
    y_7 &= \frac{4}{16}\\
    y_8 &= \frac{4}{16}\\
    y_9 &= \frac{4}{16}\\
    y_{10} &= \frac{4}{16}\\
    y_{11} &= \frac{4}{16}\\
    y_{12} &= \frac{4}{16}\\
    y_{13} &= \frac{4}{16}\\             
\end{align*}
Because this assignment exists, any optimal solution to the primal LP must have an objective value of at least $\frac{1}{4}$, showing the desired approximation ratio.

Tightness passages:
Lemma 16:
The approximation ratio of $(5+\eps)$ is tight. An instance for which this approximation ratio is achieved is given by $v_1 =\frac{1}{4}, v_2=v_3=\frac{1}{3} $ and profits of $\opt_1=\opt_L=\frac{1}{5}$ and $\opt_2=\opt_3=\frac{3}{10}.$ 
D.1 (Cardinality)
We further note that this approximation ratio is tight as well. A tight instance is given by $\opt_1=\frac{5}{17},$ $\opt_2=\opt_3=\frac{6}{17}$ with $\opt_{1\ell}=\opt_{2\ell}=\opt_{3\ell}=\frac{4}{17},$ $\opt_{1s}=\frac{1}{17}$ and $\opt_{2s}=\opt_{3s}=\frac{2}{17}.$
D.2: (Uniform profit-density)
Once again, the approximation ratio of $(4+O(\eps))$ is tight. A corresponding instance is given by $\opt_1=\opt_2=\opt_3=\opt_L=\frac{1}{4},$ with $\opt_{1\ell}=\opt_{2\ell}=\opt_{3\ell}=\opt_{Lt}=\opt_{1s}=\opt_{2s}=\opt_{3s}=\opt_{Lh}=\frac{1}{8}.$

==> omittedSec3.tex <==




\section{Omitted Proofs from \Cref{sec:structurallemma}}
\label{sec:omitted-proofs}
\subsection{Omitted Details from \Cref{sec:firstlb}}
\label{sec:omittedstrippacking}




%additional configurations using the following lemma.\mtr{Is the final figure I made meant to go here or in the appendix?}
% % \textcolor{red}{check:The small items are packed inside these regions using NFDH (note that the items in each layer are actually packed using Next-Fit-Decreasing-Depth). Again, the overshooting items are repacked into additional configurations using the following lemma.} 

% \begin{restatable}{lemma}{smallovershoot}
% \label{lem:smallovershoot}
%     The overshooting small items of any rectangular region of height $h_C$ can be repacked using \NFDH~inside a cuboid with $1\times 1$ base and height at most $O(\delta^{10})h_C + \mu$.
% \end{restatable}

% Next, note that, except possibly the rightmost rectangular region inside each arrangement, all the other regions have widths at least $\delta$. The rightmost rectangular region might not be usable as a Volume container if its width is not large enough compared to the small items
% packed in it. We consider each such region whose width is substantially small, and repack all the items packed inside the region into another configuration.

% \begin{restatable}{lemma}{smallrepack}
% \label{lem:smallrepack}
%     The small items that are packed inside the rightmost rectangular region (of an arrangement) that has width smaller than $\delta^{9}$, of a particular configuration having height $h_C$, can be repacked using \NFDH~inside a cuboid with $1\times 1$ base and height at most $O(\delta^{9})h_C+\mu$.
% \end{restatable}


% Recall that each initial configuration comprised $O(1/\delta^3)$ wide compartments, each containing $O(1/\delta^2)$ arrangements, each consisting of $1/\delta$ slots. Therefore the number of new configurations generated by Lemmas \ref{lem:wideovershoot}, \ref{lem:smallovershoot} and \ref{lem:smallrepack} is at most $O(1/\delta^6)$, and the height of each of these configurations is bounded by $O(\delta^{9})h_C+\mu$. Their total height is thus at most $O(\delta^{3})h_C + O(\mu/\delta^6) \le \epsilon h_C+O(\mu/\delta^6)$, for sufficiently small $\delta$. The increase in the height of the packing due to all these additional configurations is bounded by 
% $\epsilon\left(\frac{3}{2}+3\epsilon\right) + O\left(\frac{\mu}{\delta^6}\right)\cdot O\left(\frac{1}{\delta^6}\right) \le 2\epsilon$,
% for sufficiently small $\mu$.


% %Recall that each initial configuration comprised $O(1/\delta^3)$ wide compartments, each containing $O(1/\delta^2)$ arrangements, each consisting of $1/\delta$ slots. Therefore the number of new configurations generated by Lemmas \ref{lem:wideovershoot}, \ref{lem:smallovershoot} and \ref{lem:smallrepack} is at most $O(1/\delta^6)$, and the height of each of these configurations is bounded by $O(\delta^{c-1})h_C+\mu_s$. Their total height is thus at most $O(\delta^{c-7})h_C + O(\mu_s/\delta^6) \le \epsilon h_C+O(\mu_s/\delta^6)$, for sufficiently small $\delta$. The increase in the height of the packing due to all these additional configurations is bounded by 
% % $\epsilon\left(\frac{3}{2}+3\epsilon\right) + O\left(\frac{\mu_s}{\delta^6}\right)\cdot O\left(\frac{1}{\delta^6}\right) \le 2\epsilon$,
% % for sufficiently small $\mu_s$.

% \akr{add conditions for sufficiently small delta and mu}

% % %The number of new configurations generated due to the above lemma is at most $O(1/\delta^3)\cdot O(1/\delta^2) = O(1/\delta^5)$. We again round up the heights of these configurations to the nearest integral multiples of $\mu/\delta^{2c}$. Thus, the total (rounded) height of all the additional configurations corresponding to a configuration $C$ is bounded by 
% % \[ \left(O(\delta^c)h_C + \frac{\mu}{\delta^{2c}}\right)\cdot\frac{1}{\delta^6} + \left(O(\delta^{2c})h_C + \frac{\mu}{\delta^{2c}}\right)\cdot\frac{1}{\delta^6} + \left(O(\delta^{c-1})h_C + \frac{\mu}{\delta^{2c}}\right)\cdot \frac{1}{\delta^5} \le \epsilon h_C + O\left(\frac{1}{\delta^{2c+6}}\right)\mu \]
% % Thus, the total increase in the height of the packing due to the additional layers is at most $\epsilon(\frac{3}{2}+O(\epsilon))+O(1/\delta^{2c+6})\mu \cdot O(1/\delta^6) = O(\epsilon)$, for sufficiently small $\mu$.

% After applying Lemmas \ref{lem:wideovershoot}, \ref{lem:smallovershoot}, and \ref{lem:smallrepack}, we obtain a packing of a subset of wide and small items into containers (though their dimensions may not be from a polynomial-sized set). We now refine this packing to ensure that the container dimensions come from a \ari{set of size $n^{O(1/\delta^3)}$}. 

% \begin{restatable}{lemma}{slotsandregions}
% \label{lem:slotsandregions}
%     By losing an $O(\delta)$-fraction of the profit, the depths of all the slots for wide items and the rectangular regions for small items, can be assumed to be a multiple of $\delta^9$.
% \end{restatable}

% \ari{Analogously, we repack the long and small items inside the long compartments into such discretized slots and rectangular regions, respectively.} We note that the total number of configurations present in the current packing is $O(1/\delta^{12})$ -- there were $m=O(1/\delta^6)$ configurations to begin with, and for each initial configuration we created $O(1/\delta^6)$ additional configurations. We now round up the height of each configuration to the next integer multiple of $\mu/\epsilon$. This increases the total height by at most $\frac{\mu}{\epsilon}\cdot O\left(\frac{1}{\delta^{12}}\right) \le \epsilon$, for sufficiently small $\mu$. The resulting height of the packing is at most $(1-3\epsilon)+2\epsilon+\epsilon = 1$, and thus the packing fits inside the knapsack. Our final step is to build containers corresponding to the big compartments, slots and rectangular regions inside the configurations.


%This may not be a container packing. We now show how to obtain a container packing of the {\em overshooting} items. Recall that the height of the slot is the same as the height of the corresponding configuration.


% \wideovershoot*
% \begin{proof}
% Since the depth of the extension as well as the depth of any wide item are bounded by $\delta^{10}$, the total depth of the items not completely lying inside the original slot is at most $2\delta^{10}$. Hence it is possible to place the overshooting items of $\frac{1}{2\delta^{10}}$ \NFDH~layers, one behind the other over a $1\times 1$ square base, thus creating a single layer of items whose height is at most the maximum height of one of the $\frac{1}{2\delta^{10}}$ \NFDH~layers. Therefore the total height of the region for packing all the overshooting items of one slot is bounded by $2\delta^{10} h_C + \mu$.
% \end{proof}


% \smallovershoot*
% \begin{proof}
% The total base area of the overshooting small items of any layer is at most $4\delta^{10}$ (\ari{See Figure ??}). Hence the total base area of overshooting items of $\frac{1}{5\delta^{10}}$ layers is bounded by $4/5$, and therefore they can be packed using Next-Fit-Decreasing-Depth in one layer over a square $1\times 1$ base. The total height of all these layers is going to be at most $5\delta^{10} h_C + \mu$. This implies that the three-dimensional \NFDH~algorithm can also pack all the overshooting items within at most the same height.\mtr{I believe this should read c=10 instead of c, correct? Also, is the overshooting figure meant to be here, I dont wanna put it somewhere on a chance =)}
% \end{proof}


% \smallrepack*
% \begin{proof}
% Clearly, the base area of items packed in a single \NFDH~layer is at most $\delta^{9}$. As in the proof of \Cref{lem:smallovershoot}, we can pack all items of $\frac{1}{2\delta^{9}}$ \NFDH~layers in a single layer, from which the desired height guarantee of the lemma follows.
% \end{proof}


%\slotsandregions*
% \begin{proof}
%  We partition the compartment into strips each of depth $\delta^5$ and discard the minimum profitable strip, see \cref{fig:minStrip} for an illustration. Note that the depth of the compartment is a multiple of $\delta^4$, and hence the number of strips is at least $1/\delta$. Since each item has depth at most $\delta^{10}$, any item intersects at most two strips, and hence the total profit of the deleted items is at most an $O(\delta)$-fraction of the profit of the compartment. For any slot/rectangular region that is intersected by the deleted strip, we push the remaining items towards the front face of the slot/region, and notice that the resulting packing is again an \NFDH~packing.
    
% The resulting free space of depth $\delta^5$ inside the compartment will now be used to increase the depths of the slots and rectangular regions. Specifically, we round up the depth of each slot and region to the next integral multiple of $\delta^9$. Since the total number of slots and regions is at most $O(\frac{1}{\delta^2})\cdot O(\frac{1}{\delta}) = O(\frac{1}{\delta^3})$, the total increase in depth is bounded by $O(\frac{1}{\delta^3})\cdot \delta^9 < \delta^5$.  
% \end{proof}




% \splitconfig*
% \begin{proof}
% We construct groups of horizontal strips as follows - for $j\in [1/\epsilon]$, $\SM_j$ consists of all strips of height $\epsilon^4$ each, the distance of whose base from the base of the configuration is of the form $k\epsilon^3 + (j-1)\epsilon^4$, for some non-negative integer $k$. \ari{See Fig. ??.} Note that since $h_C$ is at most the height of the packing, which is bounded by $\frac{3}{2}+5\epsilon$, we have $k = O(1/\epsilon^3)$. Note that the height of each item packed inside the configuration is bounded by $\mu < \epsilon^4$, and therefore it intersects at most two strips. Among the $1/\epsilon$ groups of strips, we delete the group, say $\SM_{j^*}$, that intersects items of minimum profit, thereby losing only an $O(\epsilon)$-fraction of profit. This splits up the configuration into $O(1/\epsilon^3)$ new configurations, where all except possibly the bottommost and topmost configurations have height exactly $\left(\frac{1}{\epsilon}-1\right)\epsilon^3$. If $j^* \neq 1$, the bottommost configuration will have a height of $(j^*-1)\epsilon^4$. Notice that the height of the deleted strips is trivially at least $\epsilon^4$; using this free space, the height of the topmost configuration can also be made of the form $j\epsilon^4$, for some $j\in [1/\epsilon]$.
% \end{proof}


% \deleteonethird*
% \begin{proof}
% Note that the height of each configuration is at most $2\epsilon^2$ -- any configuration generated by \Cref{lem:splitconfig} has height at most $\epsilon^3$, and the remaining configurations have a height of at most $\epsilon^2 + \mu/\epsilon \le 2\epsilon^2$. We consider horizontal strips of height $7\epsilon$ each and delete all configurations intersecting the strip of minimum profit. Since each configuration intersects at most two strips, we lose only an $O(\epsilon)$-fraction of profit, and the total height of the packing now reduces to at most $\frac{3}{2}-\epsilon$. Next, we arbitrarily group the configurations into three classes, each having a total height of at most $1/2$ (note that such a grouping is always possible since the sum of the configurations' heights is at most $\frac{3}{2}-\epsilon$, and each configuration has height at most $2\epsilon^2$). Finally, we choose the two groups of largest profit and pack them inside the knapsack. Overall, we lose a profit of at most $\left(\frac{1}{3}+O(\epsilon)\right)\opt_1$.

% It remains to construct the containers from the configurations. Recall that each configuration comprises $1/\delta^2$ compartments for big items, and $O(1/\delta^3)$ compartments for packing the wide, long and small items. We create a Stack container corresponding to each of the compartments for the big items. The width (resp. depth) of this container is the same as the width (resp. depth) of some big item. Each wide compartment was further partitioned into $O(1/\delta^3)$ slots and rectangular regions, for packing the wide and small items, respectively. Note that due to \Cref{lem:slotsandregions}, the depth of an wide (resp. small) item is at most a $\delta$-fraction of the width of the slot (resp. rectangular region). Also, as a consequence of \Cref{lem:smallrepack}, the width of any small item is at most a $\delta$-fraction of the width of the region in which it is packed. Finally, the height of any configuration is at least $\text{min}\{\epsilon^4, \mu/\epsilon\} = \mu/\epsilon$, which is at least an $1/\epsilon$-factor larger than the height of any item in $I_1$. 

% We create an Area container corresponding to each slot and a Volume container for each rectangular region for the small items. The width of an Area container is the same as the width of some item in $I_1$. We note that the algorithm of \cite{3d-strip-packing} ensures that the width of a wide compartment is either a multiple of $\delta^2/2$, or a combination of the rounded widths of at most $1/\delta$ wide items. Further, the widths of the wide items are rounded up to at most $O(1/\delta^2)$ distinct values, each of which matches the width of some item in $I_1$. This results in at most $n^{O(1/\delta^3)}$ possibilities for the width of a wide compartment. Since the width of a Volume container is either the same as the width of the wide compartment or equals the difference of the width of the compartment and the width of some slot (Area container), the width of a Volume container also lies in a set of size $n^{O(1/\delta^3)}$. Finally, the heights of each of the  Stack, Area, and Volume containers are set to be same as the height of the configuration, which is an integral multiple of either $\epsilon^4$ or $\mu/\epsilon$. In a similar way, we create Area and Volume containers corresponding to the slots and rectangular regions inside the long compartments. Since there were $O(1/\delta^3)$ wide and long compartments inside the configuration to begin with, we obtain $O(1/\delta^6)$ containers overall.
% \end{proof}

\subsection{Omitted Details from \Cref{sec:5approx}}
\label{sec:sec-3-2}






\subsection{Omitted Details from \Cref{sec:secondlb}}
\label{subsec:stackLI1}








\subsection{Omitted Details from  \Cref{sec:thirdlb} and \Cref{sec:fourthlb}}
\label{sec:packI1andcombine}











% \subsection{Proof of \Cref{thm:2dknapsack}}
% \akr{Add a figure, Omitted proofs from Section 3.5?}
% Notice that since each item in $(I_2\cup L)\setminus (S_2\cup S)$ has height at least $1/2$, finding the maximum profitable packing of items in this set reduces to the two-dimensional knapsack problem where the two-dimensional items (rectangles) correspond to the top faces of the items in $(I_2\cup L)\setminus (S_2\cup S)$. Using the terminology from \cite{2dks-Lpacking}, we classify the items as large, vertical or small. Items of $L\setminus S$, having width and depth more than $\mu_l$ each, are the large items. An item $i\in I_2 \setminus S_2$ is vertical if $d_i > \mu_l$ and small if $d_i \le \mu_s$ (note that $d_i \not\in (\mu_s,\mu_l]$ since by \Cref{lem:deletemedium}, we discarded all medium items in the beginning by losing only a $\mu$-fraction of the total profit). We use the Corridor Decomposition framework of \cite{2dks-Lpacking} to obtain a packing of (a subset of) the items into corridors. The width of any corridor is at most $\mu_s$, and hence no vertical item can belong to the horizontal arms of the corridors. This implies that we can partition the corridors into containers (which will correspond to Stack and Area containers) by losing only an $O(\mu)$-fraction of profit. By a shifting argument, the total profit of items discarded during the construction of the corridors can be bounded by $O(\mu)(\beta_4+\omega_2)$. Finally, the discarded small items can be repacked into Area containers using NFDH similarly to \cite{2dks-Lpacking}, losing again an at most $O(\mu)$-fraction of profit. We make the height of each created container equal to 1.




==> other-variants.tex <==
\section{Other variants}
Using our techniques, we obtain further improvements for other variants:  (1) cardinality case (when all items have the same profit), and (2) uniform profit-density case (when the profit of an item is equal to its volume). \kvn{See \cref{sec:nonrot-cardinality,sec:nonrot-prof-eq-vol}  for the guarantees given below.}
%In the cardinality case (see \Cref{sec:nonrot-cardinality}), using standard techniques \cite{Jansencubepacking22}, we can ignore the large items in the optimal packing and obtain improved guarantees. 
%For the uniform-profit density case (see \Cref{sec:nonrot-prof-eq-vol}), we apply the volume guarantees in a more refined way. 

\begin{theorem}
    \label{thm:3dkc}
   For any constant $\eps>0$, there is a polynomial-time $(17/4 +\eps)$-approximation algorithm for \tdk~when all items have the same profit. 
\end{theorem}

\begin{theorem}
    \label{thm:3dkp}
   For any constant $\eps>0$, there is a polynomial-time $(4 +\eps)$-approximation algorithm for \tdk~when the profit of an item is equal to its volume. 
\end{theorem}

\input{variants}



\subsection{Rotational case} 
When the items can be rotated by 90 degrees around any axis, we show the existence of improved container packing. Specifically, we 
introduce a new type of container called \LContainer~and obtain improved guarantees based on the packed volume.
%We now define $f_C,\mathtt{cap}(C),\AM_C$ for an \LContainer{} $C$.

\textbf{\LContainer.} We describe \LContainers{} which ignore depth while packing the items (see \cref{fig:LContainer}; two other types of \LContainers{} exist which ignore width, height, respectively). 
%Recall that $w_C,d_C,h_C$ respectively denote the width, depth, height of $C$.
We first require that $C$ must satisfy the condition $w_C\ge h_C$.
The capacity of $C$, $\mathtt{cap}(C)$, is given by $w_Ch_C-w_C^2/4$ (see \cref{pack-sheets} in \cref{sec:Lcontainer}).
For each item $i$ packed inside $C$, \kvn{there must be some orientation with} width at least $w_C/2$, depth at least $d_C/2$, and height at most $\eps h_C$.
If these conditions are satisfied, then we set $f_C(i)\coloneqq w_ih_i$ and $\infty$ otherwise.
Algorithm $\AM_C$ is as follows. Given a set of items $T$ satisfying $f_C(T)\le \mathtt{cap}(C)$, we arrange them in non-increasing order of profit/front area ratio.
Then, we select the largest prefix $T'$ whose total front area does not exceed $w_Ch_C-w_C^2/4-3\eps h_C^2$. We now sort the items in $T'$
in non-increasing order of \kvn{widths}, start from the bottom left corner, and keep stacking them one upon each other to the maximum extent possible.
Then, we rotate the remaining items by $90$ degrees around the depth axis, start from the top right corner and keep packing them side by side.
(See \cref{pack-sheets} in \cref{sec:Lcontainer}.)

The main ingredient to obtain improved approximation ratios in the rotational case is our algorithm \texttt{3DR-Vol-Pack} (see \Cref{sec:subroutines}). However as stated, the algorithm does not pack items into (guessable) containers. We show in \Cref{sec:3dr-vol-pack} that the algorithm can be modified to return a guessable container packing into Stack, Steinberg, and $\mathsf{L}$-Containers. Using this, we obtain the following theorems for the general case, cardinality case, and uniform profit-density case. See \cref{sec:rot-general-case,sec:tdkrc,sec:tdkrp} for the respective proofs.

%In this case, our main result is the following.

\begin{figure}
    \centering
    \includesvg[width=0.5\linewidth]{img/L-container.svg}
    \caption{An example packing of items inside an \LContainer.}
    \label{fig:LContainer}
\end{figure}
% \begin{lemma}
%     Let $T$ be a set of items such that each $i\in T$ has at least one of the dimensions not exceeding $\epsilon$. If $v(T) \le \frac{7}{24}-5\epsilon$, then there exists a partition $T = T_{\ell} \dot{\cup} T_s$, such that items of $T_s$ can be packed into a Steinberg container, and items of $T_{\ell}$ can be packed into either an \LContainer~or a Stack container. Further, the heights of the containers are integral multiples of $\epsilon^2$.
% \end{lemma}



% Using the above lemma, we obtain the following theorems for the general case, cardinality case, and the case when profit equals volume for each item. See \cref{sec:rot-general-case,sec:tdkrc,sec:tdkrp} for the respective proofs.
\begin{theorem}
    \label{thm:3dkrot}
   For any constant $\eps>0$, there is a polynomial-time $(30/7+\eps)$-approximation algorithm for \tdkr. 
\end{theorem}

\begin{theorem}
    \label{thm:r3dkce}
   For any constant $\eps>0$, there is a polynomial-time $(24/7 +\eps)$-approximation algorithm for \tdkr~when all items have the same profit.  
\end{theorem}

\begin{restatable}{theorem}{profitequalsvolrot}
    \label{thm:r3dkrp}
   For any constant $\eps>0$, there is a polynomial-time $(3 +\eps)$-approximation algorithm for \tdkr~when the profit of an item is equal to its volume.  
\end{restatable}


\section{Conclusion}
%We showed improved approximation guarantees for \tdk. 
In this work, our primary focus has been to obtain improved polynomial-time approximation guarantees. %We did not try to optimize the runtime. 
\kvn{Our current runtime of $n^{f(1/\eps)}$ is mainly because of the step where we guess the containers and assign the items. Once this is done,
every $\AM_C$ runs in time $O(n\log^2 n)$. Hence, one interesting direction is whether the time to guess the containers and assign the items can be brought down to $(n \cdot (\log n)^{f(1/\eps)})$ using the recent 
techniques of \cite{BuchemDW24}.}
% One interesting open question is whether it is possible to obtain near-linear runtime $(n \cdot (\log n)^{f(1/\eps)})$ from our present runtime of $n^{f(1/\eps)}$ using the recent techniques from \cite{BuchemDW24}. 
Another interesting open problem is to provide a tight approximation for algorithms based on container packing.

 

